Energy-based Hopfield Boosting for Out-of-Distribution Detection

Out-of-distribution (OOD) detection is critical when deploying machine learning models in the real world. Outlier exposure methods, which incorporate auxiliary outlier data in the training process, can drastically improve OOD detection performance compared to approaches without advanced training strategies. We introduce Hopfield Boosting, a boosting approach, which leverages modern Hopfield energy (MHE) to sharpen the decision boundary between the in-distribution and OOD data. Hopfield Boosting encourages the model to concentrate on hard-to-distinguish auxiliary outlier examples that lie close to the decision boundary between in-distribution and auxiliary outlier data. Our method achieves a new state-of-the-art in OOD detection with outlier exposure, improving the FPR95 metric from 2.28 to 0.92 on CIFAR-10 and from 11.76 to 7.94 on CIFAR-100.

==> tables/ablation_sampling.tex <==
\begin{table*}[t]
\centering
\caption{
OOD detection performance on CIFAR-10. We compare \ourmethod trained with weighted sampling and random sampling on ResNet-18. $\downarrow$ indicates ``lower is better'' and $\uparrow$ indicates ``higher is better''. All values in $\%$. Standard deviations are estimated across five training runs.}%
\label{tab:sampling_ablation}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{l|ll|ll}
 & \multicolumn{2}{c}{Weighted Sampling} & \multicolumn{2}{c}{Random Sampling}\\
 OOD Dataset  & \text{FPR95 } $\downarrow$ & \text{AUROC } $\uparrow$ & \text{FPR95 } $\downarrow$ & \text{AUROC } $\uparrow$ \\
\midrule
\rowcolor{gray!25}
 \text{SVHN} & $\mathbf{0.23 ^ {\pm 0.08}}$  & $\mathbf{99.57 ^ {\pm 0.06}}$ &
               $0.70 ^ {\pm 0.13}$ & $\mathbf{99.55 ^ {\pm 0.08}}$ \\
 \text{LSUN-Crop} & $\mathbf{0.82 ^ {\pm 0.20}}$ & $\mathbf{99.40 ^ {\pm 0.05}}$ &
                    $1.58 ^ {\pm 0.31}$  & $99.24 ^ {\pm 0.10}$ \\
\rowcolor{gray!25}
 \text{LSUN-Resize} & $\mathbf{0.00 ^ {\pm 0.00}}$ & $\mathbf{99.98 ^ {\pm 0.02}}$ & 
                    $ \mathbf{0.00 ^ {\pm 0.00}}$  & $\mathbf{99.98 ^ {\pm 0.01}}$  \\
 \text{Textures} & $\mathbf{0.16 ^ {\pm 0.02}}$ & $\mathbf{99.85 ^ {\pm 0.01}}$ &
                   $ 0.26^ {\pm 0.06}$ & $99.81 ^ {\pm 0.02}$ \\
\rowcolor{gray!25}
 \text{iSUN} & $\mathbf{0.00 ^ {\pm 0.00}}$ & $99.97 ^ {\pm 0.02}$ &
                $ \mathbf{0.00 ^ {\pm 0.00}}$ & $\mathbf{99.99 ^ {\pm 0.00}}$ \\
\text{Places 365} & $\mathbf{4.28 ^ {\pm 0.26}}$ & $\mathbf{98.51 ^ {\pm 0.11}}$ &
                    $6.20 ^ {\pm 0.21} $ & $97.68 ^ {\pm 0.21}$ \\

\midrule



 \textbf{Mean} & $\mathbf{0.92}$ & $\mathbf{99.55}$
                & $1.46$ & $99.38$\\

\end{tabular}}
\end{table*}

